A Catalog of Calibrator Stars for Next-Generation Optical Interferometers

Benchmark stars with known angular diameters are key to calibrating interferometric observations. With the advent of optical interferometry, there is a need for suitably bright, well-vetted calibrator stars over a large portion of the sky. We present a catalog of uniformly computed angular diameters for 1523 stars in the northern hemisphere brighter than V = 6 and with declinations $-15^\circ < \delta < 82^\circ$. The median angular stellar diameter is 0.527 mas. The list has been carefully cleansed of all known binary and multiple stellar systems. We derive the angular diameters for each of the stars by fitting spectral templates to the observed spectral energy distributions (SEDs) from literature fluxes. We compare these derived angular diameters against those measured by optical interferometry for 75 of the stars, as well as to 176 diameter estimates from previous calibrator catalogs, finding in general excellent agreement. The final catalog includes our goodness-of-fit metrics as well as an online atlas of our SED fits. The catalog presented here permits selection of the best calibrator stars for current and future visible-light interferometric observations.

==> report.tex <==
@ARTICLE{Mermilliod1997,
   author = {{Mermilliod}, J.-C. and {Mermilliod}, M. and {Hauck}, B.},
    title = "{The General Catalogue of Photometric Data (GCPD). II.}",
  journal = {\aaps},
 keywords = {CATALOGUES, STARS: GENERAL, TECHNIQUES: PHOTOMETRIC},
     year = 1997,
    month = aug,
   volume = 124,
    pages = {349-352},
      doi = {10.1051/aas:1997197},
   adsurl = {http://adsabs.harvard.edu/abs/1997A\%26AS..124..349M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Richichi09,
   author = {{Richichi}, A. and {Percheron}, I. and {Davis}, J.},
    title = "{A list of bright interferometric calibrators measured at the European Southern Observatory Very Large Telescope Interferometer}",
  journal = {\mnras},
 keywords = {techniques: high angular resolution , techniques: interferometric , catalogues , stars: fundamental parameters},
     year = 2009,
    month = oct,
   volume = 399,
    pages = {399-409},
      doi = {10.1111/j.1365-2966.2009.15289.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009MNRAS.399..399R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia16,
   author = {{Garcia}, E.~V. and {Muterspaugh}, M.~W. and {van Belle}, G. and 
	{Monnier}, J.~D. and {Stassun}, K.~G. and {Ghasempour}, A. and 
	{Clark}, J.~H. and {Zavala}, R.~T. and {Benson}, J.~A. and {Hutter}, D.~J. and 
	{Schmitt}, H.~R. and {Baines}, E.~K. and {Jorgensen}, A.~M. and 
	{Strosahl}, S.~G. and {Sanborn}, J. and {Zawicki}, S.~J. and 
	{Sakosky}, M.~F. and {Swihart}, S.},
    title = "{Vision: A Six-telescope Fiber-fed Visible Light Beam Combiner for the Navy Precision Optical Interferometer}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1601.00036},
 primaryClass = "astro-ph.IM",
     year = 2016,
    month = may,
   volume = 128,
   number = 5,
    pages = {055004},
      doi = {10.1088/1538-3873/128/963/055004},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016PASP..128e5004G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Press02,
   author = {{Press}, W.~H. and {Teukolsky}, S.~A. and {Vetterling}, W.~T. and 
	{Flannery}, B.~P.},
    title = "{Numerical recipes in C++ : the art of scientific computing}",
booktitle = {Numerical recipes in C++ : the art of scientific computing by William H.~Press.~xxviii, 1,002 p.~: ill.~; 26 cm.~ Includes bibliographical references and index.~ISBN :  0521750334},
     year = 2002,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002nrca.book.....P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Andrae10,
   author = {{Andrae}, R. and {Schulze-Hartung}, T. and {Melchior}, P.},
    title = "{Dos and don'ts of reduced chi-squared}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1012.3754},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Data Analysis, Statistics and Probability, Statistics - Methodology},
     year = 2010,
    month = dec,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010arXiv1012.3754A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Boggess78,
   author = {{Boggess}, A. and {Carr}, F.~A. and {Evans}, D.~C. and {Fischel}, D. and 
	{Freeman}, H.~R. and {Fuechsel}, C.~F. and {Klinglesmith}, D.~A. and 
	{Krueger}, V.~L. and {Longanecker}, G.~W. and {Moore}, J.~V.
	},
    title = "{The IUE spacecraft and instrumentation}",
  journal = {\nat},
 keywords = {Ground Based Control, Iue, Satellite Design, Satellite-Borne Instruments, Spaceborne Astronomy, Spacecraft Communication, Ultraviolet Astronomy, Explorer Satellites, Satellite Antennas, Satellite-Borne Photography, Solar Arrays, Ultraviolet Photography},
     year = 1978,
    month = oct,
   volume = 275,
    pages = {372-377},
      doi = {10.1038/275372a0},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1978Natur.275..372B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2MASSsys,
   author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and 
	{Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and 
	{Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and 
	{Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and 
	{Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and 
	{Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and 
	{Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and 
	{Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and 
	{Wheelock}, S.},
    title = "{The Two Micron All Sky Survey (2MASS)}",
  journal = {\aj},
 keywords = {Catalogs, Infrared: General, Surveys},
     year = 2006,
    month = feb,
   volume = 131,
    pages = {1163-1183},
      doi = {10.1086/498708},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006AJ....131.1163S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@PROCEEDINGS{IrasSys,
    title = "{Infrared astronomical satellite (IRAS) catalogs and atlases. Volume 1: Explanatory supplement}",
 keywords = {All Sky Photography, Catalogs, Indexes (Documentation), Infrared Astronomy Satellite, Cosmology, Galaxies, Star Formation, Stellar Evolution},
booktitle = {Infrared astronomical satellite (IRAS) catalogs and atlases. Volume 1: Explanatory supplement},
     year = 1988,
   volume = 1,
   editor = {{Beichman}, C.~A. and {Neugebauer}, G. and {Habing}, H.~J. and 
	{Clegg}, P.~E. and {Chester}, T.~J.},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1988iras....1.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ViliniusSys,
   author = {{North}, P.},
    title = "{Vilnius Photometric Catalogue}",
  journal = {\aaps},
     year = 1980,
    month = sep,
   volume = 41,
    pages = {395},
   adsurl = {http://adsabs.harvard.edu/abs/1980A%26AS...41..395N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ThirteenSys,
   author = {{Johnson}, H.~L. and {Mitchell}, R.~I.},
    title = "{Thirteen-color photometry of 1380 bright stars.}",
  journal = {\rmxaa},
     year = 1975,
    month = sep,
   volume = 1,
    pages = {299-324},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1975RMxAA...1..299J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{GenevaSys,
   author = {{Golay}, M.},
    title = "{Spectral classification through seven-colour photometry}",
  journal = {Vistas in Astronomy},
     year = 1972,
   volume = 14,
    pages = {13-51},
      doi = {10.1016/0083-6656(72)90023-2},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1972VA.....14...13G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{StromSys,
   author = {{Str{\"o}mgren}, B.},
    title = "{Two-dimensional spectral classification of F stars through photoelectric photometry with interference filters}",
  journal = {Vistas in Astronomy},
     year = 1956,
   volume = 2,
    pages = {1336-1346},
      doi = {10.1016/0083-6656(56)90060-5},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1956VA......2.1336S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DDOsys,
   author = {{McClure}, R.~D.},
    title = "{Standard stars for DDO photometry.}",
  journal = {\aj},
     year = 1976,
    month = mar,
   volume = 81,
    pages = {182-208},
      doi = {10.1086/111873},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1976AJ.....81..182M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{JohnsonSys,
   author = {{Johnson}, H.~L. and {Morgan}, W.~W.},
    title = "{Fundamental stellar photometry for standards of spectral type on the revised system of the Yerkes spectral atlas}",
  journal = {\apj},
     year = 1953,
    month = may,
   volume = 117,
    pages = {313},
      doi = {10.1086/145697},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1953ApJ...117..313J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Simbad,
   author = {{Wenger}, M. and {Ochsenbein}, F. and {Egret}, D. and {Dubois}, P. and 
	{Bonnarel}, F. and {Borde}, S. and {Genova}, F. and {Jasniewicz}, G. and 
	{Lalo{\"e}}, S. and {Lesteven}, S. and {Monier}, R.},
    title = "{The SIMBAD astronomical database. The CDS reference database for astronomical objects}",
  journal = {\aaps},
   eprint = {astro-ph/0002110},
 keywords = {ASTRONOMICAL DATA BASES: MISCELLANEOUS, CATALOGS},
     year = 2000,
    month = apr,
   volume = 143,
    pages = {9-22},
      doi = {10.1051/aas:2000332},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26AS..143....9W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pickles98,
   author = {{Pickles}, A.~J.},
    title = "{A Stellar Spectral Flux Library: 1150-25000 {\AA}}",
  journal = {\pasp},
 keywords = {ATLASES, STARS: GENERAL, GALAXIES: STELLAR CONTENT},
     year = 1998,
    month = jul,
   volume = 110,
    pages = {863-878},
      doi = {10.1086/316197},
   adsurl = {http://adsabs.harvard.edu/abs/1998PASP..110..863P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SB9,
   author = {{Pourbaix}, D. and {Tokovinin}, A.~A. and {Batten}, A.~H. and 
	{Fekel}, F.~C. and {Hartkopf}, W.~I. and {Levato}, H. and {Morrell}, N.~I. and 
	{Torres}, G. and {Udry}, S.},
    title = "{S$_{B<SUP>9</SUP>}$: The ninth catalogue of spectroscopic binary orbits}",
  journal = {\aap},
   eprint = {astro-ph/0406573},
 keywords = {stars: binaries: spectroscopic, astronomical data bases: miscellaneous, catalogs},
     year = 2004,
    month = sep,
   volume = 424,
    pages = {727-732},
      doi = {10.1051/0004-6361:20041213},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...424..727P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{WDS,
   author = {{Mason}, B.~D. and {Wycoff}, G.~L. and {Hartkopf}, W.~I. and 
	{Douglass}, G.~G. and {Worley}, C.~E.},
    title = "{The 2001 US Naval Observatory Double Star CD-ROM. I. The Washington Double Star Catalog}",
  journal = {\aj},
 keywords = {Stars: Binaries: General, Stars: Binaries: Visual, Catalogs},
     year = 2001,
    month = dec,
   volume = 122,
    pages = {3466-3471},
      doi = {10.1086/323920},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122.3466M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{skiff,
   author = {{Skiff}, B.~A.},
    title = "{VizieR Online Data Catalog: Catalogue of stellar spectral classifications.}",
  journal = {VizieR Online Data Catalog},
     year = 2009,
   volume = 1,
    pages = {2023},
   adsurl = {http://adsabs.harvard.edu/abs/2009yCat....1.2023S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boyajian2012B,
   author = {{Boyajian}, T.~S. and {von Braun}, K. and {van Belle}, G. and 
	{McAlister}, H.~A. and {ten Brummelaar}, T.~A. and {Kane}, S.~R. and 
	{Muirhead}, P.~S. and {Jones}, J. and {White}, R. and {Schaefer}, G. and 
	{Ciardi}, D. and {Henry}, T. and {L{\'o}pez-Morales}, M. and 
	{Ridgway}, S. and {Gies}, D. and {Jao}, W.-C. and {Rojas-Ayala}, B. and 
	{Parks}, J.~R. and {Sturmann}, L. and {Sturmann}, J. and {Turner}, N.~H. and 
	{Farrington}, C. and {Goldfinger}, P.~J. and {Berger}, D.~H.
	},
    title = "{Stellar Diameters and Temperatures. II. Main-sequence K- and M-stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1208.2431},
 primaryClass = "astro-ph.SR",
 keywords = {Hertzsprung-Russell and C-M diagrams, infrared: stars, planetary systems, stars: atmospheres, stars: fundamental parameters, stars: general, stars: late-type, stars: low-mass, techniques: high angular resolution, techniques: interferometric},
     year = 2012,
    month = oct,
   volume = 757,
      eid = {112},
    pages = {112},
      doi = {10.1088/0004-637X/757/2/112},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boyajian2012A,
   author = {{Boyajian}, T.~S. and {McAlister}, H.~A. and {van Belle}, G. and 
	{Gies}, D.~R. and {ten Brummelaar}, T.~A. and {von Braun}, K. and 
	{Farrington}, C. and {Goldfinger}, P.~J. and {O'Brien}, D. and 
	{Parks}, J.~R. and {Richardson}, N.~D. and {Ridgway}, S. and 
	{Schaefer}, G. and {Sturmann}, L. and {Sturmann}, J. and {Touhami}, Y. and 
	{Turner}, N.~H. and {White}, R.},
    title = "{Stellar Diameters and Temperatures. I. Main-sequence A, F, and G Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.3316},
 primaryClass = "astro-ph.SR",
 keywords = {Hertzsprung-Russell and C-M diagrams, infrared: stars, stars: evolution, stars: fundamental parameters, stars: late-type, stars: solar-type, techniques: interferometric},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {101},
    pages = {101},
      doi = {10.1088/0004-637X/746/1/101},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...746..101B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boyajian2013,
   author = {{Boyajian}, T.~S. and {von Braun}, K. and {van Belle}, G. and 
	{Farrington}, C. and {Schaefer}, G. and {Jones}, J. and {White}, R. and 
	{McAlister}, H.~A. and {ten Brummelaar}, T.~A. and {Ridgway}, S. and 
	{Gies}, D. and {Sturmann}, L. and {Sturmann}, J. and {Turner}, N.~H. and 
	{Goldfinger}, P.~J. and {Vargas}, N.},
    title = "{Stellar Diameters and Temperatures. III. Main-sequence A, F, G, and K Stars: Additional High-precision Measurements and Empirical Relations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1306.2974},
 primaryClass = "astro-ph.SR",
 keywords = {Hertzsprung-Russell and C-M diagrams, infrared: stars, planetary systems, stars: atmospheres, stars: fundamental parameters, stars: general, stars: solar-type, techniques: high angular resolution, techniques: interferometric},
     year = 2013,
    month = jul,
   volume = 771,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/771/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...771...40B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{NPOI,
   author = {{Armstrong}, J.~T. and {Mozurkewich}, D. and {Rickard}, L.~J. and 
	{Hutter}, D.~J. and {Benson}, J.~A. and {Bowers}, P.~F. and 
	{Elias}, II, N.~M. and {Hummel}, C.~A. and {Johnston}, K.~J. and 
	{Buscher}, D.~F. and {Clark}, III, J.~H. and {Ha}, L. and {Ling}, L.-C. and 
	{White}, N.~M. and {Simon}, R.~S.},
    title = "{The Navy Prototype Optical Interferometer}",
  journal = {\apj},
 keywords = {INSTRUMENTATION: INTERFEROMETERS, TECHNIQUES: INTERFEROMETRIC, Instrumentation: Interferometers, Techniques: Interferometric},
     year = 1998,
    month = mar,
   volume = 496,
    pages = {550-571},
      doi = {10.1086/305365},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1998ApJ...496..550A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{CHARA,
   author = {{ten Brummelaar}, T.~A. and {McAlister}, H.~A. and {Ridgway}, S.~T. and 
	{Bagnuolo}, Jr., W.~G. and {Turner}, N.~H. and {Sturmann}, L. and 
	{Sturmann}, J. and {Berger}, D.~H. and {Ogden}, C.~E. and {Cadman}, R. and 
	{Hartkopf}, W.~I. and {Hopper}, C.~H. and {Shure}, M.~A.},
    title = "{First Results from the CHARA Array. II. A Description of the Instrument}",
  journal = {\apj},
   eprint = {astro-ph/0504082},
 keywords = {Atmospheric Effects, Instrumentation: High Angular Resolution, Instrumentation: Interferometers, Techniques: High Anular Resolution, Techniques: Interferometric, Telescopes},
     year = 2005,
    month = jul,
   volume = 628,
    pages = {453-465},
      doi = {10.1086/430729},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...628..453T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{vanBellevanBelle05,
   author = {{van Belle}, G.~T. and {van Belle}, G.},
    title = "{Establishing Visible Interferometer System Responses: Resolved and Unresolved Calibrators}",
  journal = {\pasp},
   eprint = {astro-ph/0508266},
 keywords = {Instrumentation: Interferometers, Methods: Analytical, Techniques: Interferometric, Stars: Fundamental Parameters},
     year = 2005,
    month = nov,
   volume = 117,
    pages = {1263-1270},
      doi = {10.1086/449603},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005PASP..117.1263V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{challouf,
   author = {{Challouf}, M. and {Nardetto}, N. and {Mourard}, D. and {Aroui}, H. and 
	{Delaa}, O.},
    title = "{Measurements of eight early-type stars angular diameters using VEGA/CHARA interferometer}",
 keywords = {Stars: early-type, methods: data analysis, instrumentation: interferometers, techniques: medium spectral resolution},
booktitle = {SF2A-2014: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics},
     year = 2014,
   editor = {{Ballet}, J. and {Martins}, F. and {Bournaud}, F. and {Monier}, R. and 
	{Reyl{\'e}}, C.},
    month = dec,
    pages = {471-474},
   adsurl = {http://adsabs.harvard.edu/abs/2014sf2a.conf..471C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maestro13,
   author = {{Maestro}, V. and {Che}, X. and {Huber}, D. and {Ireland}, M.~J. and 
	{Monnier}, J.~D. and {White}, T.~R. and {Kok}, Y. and {Robertson}, J.~G. and 
	{Schaefer}, G.~H. and {ten Brummelaar}, T.~A. and {Tuthill}, P.~G.
	},
    title = "{Optical interferometry of early-type stars with PAVO@CHARA - I. Fundamental stellar properties}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1306.5937},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: interferometric, stars: early-type, stars: fundamental parameters},
     year = 2013,
    month = sep,
   volume = 434,
    pages = {1321-1331},
      doi = {10.1093/mnras/stt1092},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.434.1321M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eggleton08,
   author = {{Eggleton}, P.~P. and {Tokovinin}, A.~A.},
    title = "{A catalogue of multiplicity among bright stellar systems}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.2878},
 keywords = {binaries: close , stars: statistics},
     year = 2008,
    month = sep,
   volume = 389,
    pages = {869-879},
      doi = {10.1111/j.1365-2966.2008.13596.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008MNRAS.389..869E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanLeeuwen07,
   author = {{van Leeuwen}, F.},
    title = "{Validation of the new Hipparcos reduction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0708.1752},
 keywords = {space vehicles: instruments, methods: data analysis, catalogs, astrometry, instrumentation: miscellaneous},
     year = 2007,
    month = nov,
   volume = 474,
    pages = {653-664},
      doi = {10.1051/0004-6361:20078357},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...474..653V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{CLIMBcomb,
   author = {{ten Brummelaar}, T.~A. and {Sturmann}, J. and {Ridgway}, S.~T. and 
	{Sturmann}, L. and {Turner}, N.~H. and {McAlister}, H.~A. and 
	{Farrington}, C.~D. and {Beckmann}, U. and {Weigelt}, G. and 
	{Shure}, M.},
    title = "{The Classic/climb Beam Combiner at the CHARA Array}",
  journal = {Journal of Astronomical Instrumentation },
 keywords = {Interferometry, beam combiner, closure phase, imaging, visibility, detector},
     year = 2013,
   volume = 2,
      eid = {1340004},
    pages = {40004},
      doi = {10.1142/S2251171713400047},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013JAI.....240004T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{VEGAcomb,
   author = {{Mourard}, D. and {Clausse}, J.~M. and {Marcotto}, A. and {Perraut}, K. and 
	{Tallon-Bosc}, I. and {B{\'e}rio}, P. and {Blazit}, A. and {Bonneau}, D. and 
	{Bosio}, S. and {Bresson}, Y. and {Chesneau}, O. and {Delaa}, O. and 
	{H{\'e}nault}, F. and {Hughes}, Y. and {Lagarde}, S. and {Merlin}, G. and 
	{Roussel}, A. and {Spang}, A. and {Stee}, P. and {Tallon}, M. and 
	{Antonelli}, P. and {Foy}, R. and {Kervella}, P. and {Petrov}, R. and 
	{Thiebaut}, E. and {Vakili}, F. and {McAlister}, H. and {ten Brummelaar}, T. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N. and {Farrington}, C. and 
	{Goldfinger}, P.~J.},
    title = "{VEGA: Visible spEctroGraph and polArimeter for the CHARA array: principle and performance}",
  journal = {\aap},
 keywords = {instrumentation: high angular resolution, instrumentation: interferometers},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {1073-1083},
      doi = {10.1051/0004-6361/200913016},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009A%26A...508.1073M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{PAVOcomb,
   author = {{Ireland}, M.~J. and {M{\'e}rand}, A. and {ten Brummelaar}, T.~A. and 
	{Tuthill}, P.~G. and {Schaefer}, G.~H. and {Turner}, N.~H. and 
	{Sturmann}, J. and {Sturmann}, L. and {McAlister}, H.~A.},
    title = "{Sensitive visible interferometry with PAVO}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2008,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 7013,
    month = jul,
      eid = {701324},
    pages = {24},
      doi = {10.1117/12.788386},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008SPIE.7013E..24I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{MIRCcomb,
   author = {{Monnier}, J.~D. and {Berger}, J.-P. and {Millan-Gabet}, R. and 
	{ten Brummelaar}, T.~A.},
    title = "{The Michigan Infrared Combiner (MIRC): IR imaging with the CHARA Array}",
booktitle = {New Frontiers in Stellar Interferometry},
     year = 2004,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 5491,
   editor = {{Traub}, W.~A.},
    month = oct,
    pages = {1370},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004SPIE.5491.1370M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Ghasempour12,
   author = {{Ghasempour}, A. and {Muterspaugh}, M.~W. and {Hutter}, D.~J. and 
	{Monnier}, J.~D. and {Benson}, J.~A. and {Armstrong}, J.~T. and 
	{Williamson}, M.~H. and {Fall}, S. and {Harrison}, C. and {Sergeyous}, C.
	},
    title = "{Building the next-generation science camera for the Navy Optical Interferometer}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2012,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 8445,
    month = jul,
      eid = {84450M},
    pages = {0},
      doi = {10.1117/12.924995},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012SPIE.8445E..0MG},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ligi12,
   author = {{Ligi}, R. and {Mourard}, D. and {Lagrange}, A.~M. and {Perraut}, K. and 
	{Boyajian}, T. and {B{\'e}rio}, P. and {Nardetto}, N. and {Tallon-Bosc}, I. and 
	{McAlister}, H. and {ten Brummelaar}, T. and {Ridgway}, S. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N. and {Farrington}, C. and 
	{Goldfinger}, P.~J.},
    title = "{A new interferometric study of four exoplanet host stars: {$\theta$} Cygni, 14 Andromedae, {$\upsilon$} Andromedae and 42 Draconis}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1208.3895},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters, methods: data analysis, techniques: high angular resolution, instrumentation: interferometers},
     year = 2012,
    month = sep,
   volume = 545,
      eid = {A5},
    pages = {A5},
      doi = {10.1051/0004-6361/201219467},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...545A...5L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mozurkewich03,
   author = {{Mozurkewich}, D. and {Armstrong}, J.~T. and {Hindsley}, R.~B. and 
	{Quirrenbach}, A. and {Hummel}, C.~A. and {Hutter}, D.~J. and 
	{Johnston}, K.~J. and {Hajian}, A.~R. and {Elias}, II, N.~M. and 
	{Buscher}, D.~F. and {Simon}, R.~S.},
    title = "{Angular Diameters of Stars from the Mark III Optical Interferometer}",
  journal = {\aj},
 keywords = {Stars: Atmospheres, Stars: Fundamental Parameters},
     year = 2003,
    month = nov,
   volume = 126,
    pages = {2502-2520},
      doi = {10.1086/378596},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2003AJ....126.2502M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{massa84,
   author = {{Massa}, D. and {Savage}, B.~D.},
    title = "{Ultraviolet observations of interstellar extinction near the Cepheus OB3 molecular cloud}",
  journal = {\apj},
 keywords = {Interstellar Extinction, Interstellar Matter, Iue, Molecular Clouds, Ultraviolet Astronomy, B Stars, Carbon Monoxide, Early Stars, O Stars, Stellar Spectra, Stellar Spectrophotometry},
     year = 1984,
    month = apr,
   volume = 279,
    pages = {310-321},
      doi = {10.1086/161892},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1984ApJ...279..310M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{massa81,
   author = {{Massa}, D. and {Conti}, P.~S.},
    title = "{IUE observations of eight OB stars in NGC 2244 - Ultraviolet continua and extinction}",
  journal = {\apj},
 keywords = {Early Stars, Interstellar Extinction, Interstellar Matter, Iue, Stellar Spectrophotometry, Ultraviolet Astronomy, B Stars, O Stars, Open Clusters, Stellar Atmospheres, Stellar Magnitude, Stellar Spectra},
     year = 1981,
    month = aug,
   volume = 248,
    pages = {201-213},
      doi = {10.1086/159144},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1981ApJ...248..201M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanBelle16,
   author = {{van Belle}, G.~T. and {Creech-Eakman}, M. and {Ruiz-Velasco}, A.
	},
    title = "{Bolometric Flux Estimation for Cool Evolved Stars}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1604.00984},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2016,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160400984V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanBelle09,
   author = {{van Belle}, G.~T. and {von Braun}, K.},
    title = "{Directly Determined Linear Radii and Effective Temperatures of Exoplanet Host Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0901.1206},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, stars: fundamental parameters, techniques: interferometric},
     year = 2009,
    month = apr,
   volume = 694,
    pages = {1085-1098},
      doi = {10.1088/0004-637X/694/2/1085},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009ApJ...694.1085V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Braun14,
   author = {{von Braun}, K. and {Boyajian}, T.~S. and {van Belle}, G.~T. and 
	{Kane}, S.~R. and {Jones}, J. and {Farrington}, C. and {Schaefer}, G. and 
	{Vargas}, N. and {Scott}, N. and {ten Brummelaar}, T.~A. and 
	{Kephart}, M. and {Gies}, D.~R. and {Ciardi}, D.~R. and {L{\'o}pez-Morales}, M. and 
	{Mazingue}, C. and {McAlister}, H.~A. and {Ridgway}, S. and 
	{Goldfinger}, P.~J. and {Turner}, N.~H. and {Sturmann}, L.},
    title = "{Stellar diameters and temperatures - V. 11 newly characterized exoplanet host stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1312.1792},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: interferometric, stars: fundamental parameters, stars: general, stars: late-type, planetary systems, infrared: stars},
     year = 2014,
    month = mar,
   volume = 438,
    pages = {2413-2425},
      doi = {10.1093/mnras/stt2360},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.2413V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baines09,
   author = {{Baines}, E.~K. and {McAlister}, H.~A. and {ten Brummelaar}, T.~A. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N.~H. and {Ridgway}, S.~T.
	},
    title = "{Eleven Exoplanet Host Star Angular Diameters from the Chara Array}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0906.2702},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, planetary systems, stars: fundamental parameters, techniques: interferometric},
     year = 2009,
    month = aug,
   volume = 701,
    pages = {154-162},
      doi = {10.1088/0004-637X/701/1/154},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...701..154B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boyajian09,
   author = {{Boyajian}, T.~S. and {McAlister}, H.~A. and {Cantrell}, J.~R. and 
	{Gies}, D.~R. and {ten Brummelaar}, T.~A. and {Farrington}, C. and 
	{Goldfinger}, P.~J. and {Sturmann}, L. and {Sturmann}, J. and 
	{Turner}, N.~H. and {Ridgway}, S.},
    title = "{Angular Diameters of the Hyades Giants Measured with the CHARA Array}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0810.2238},
 keywords = {infrared: stars, stars: fundamental parameters, techniques: interferometric},
     year = 2009,
    month = feb,
   volume = 691,
    pages = {1243-1247},
      doi = {10.1088/0004-637X/691/2/1243},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691.1243B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baines10,
   author = {{Baines}, E.~K. and {D{\"o}llinger}, M.~P. and {Cusano}, F. and 
	{Guenther}, E.~W. and {Hatzes}, A.~P. and {McAlister}, H.~A. and 
	{ten Brummelaar}, T.~A. and {Turner}, N.~H. and {Sturmann}, J. and 
	{Sturmann}, L. and {Goldfinger}, P.~J. and {Farrington}, C.~D. and 
	{Ridgway}, S.~T.},
    title = "{Angular Diameters and Effective Temperatures of 25 K Giant Stars from the CHARA Array}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0912.5491},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, planetary systems, stars: fundamental parameters, techniques: interferometric, techniques: spectroscopic},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {1365-1374},
      doi = {10.1088/0004-637X/710/2/1365},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710.1365B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{STELIB,
   author = {{Le Borgne}, J.-F. and {Bruzual}, G. and {Pell{\'o}}, R. and 
	{Lan{\c c}on}, A. and {Rocca-Volmerange}, B. and {Sanahuja}, B. and 
	{Schaerer}, D. and {Soubiran}, C. and {V{\'{\i}}lchez-G{\'o}mez}, R.
	},
    title = "{STELIB: A library of stellar spectra at R \~{} 2000}",
  journal = {\aap},
   eprint = {astro-ph/0302334},
 keywords = {atlases, stars: fundamental parameters, galaxies: stellar content.},
     year = 2003,
    month = may,
   volume = 402,
    pages = {433-442},
      doi = {10.1051/0004-6361:20030243},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...402..433L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Borde:2002,
   author = {{Bord{\'e}}, P. and {Coud{\'e} du Foresto}, V. and {Chagnon}, G. and 
	{Perrin}, G.},
    title = "{A catalogue of calibrator stars for long baseline stellar interferometry}",
  journal = {\aap},
 keywords = {catalogs, stars: fundamental parameters, instrumentation: interferometers, techniques: interferometric},
     year = 2002,
    month = oct,
   volume = 393,
    pages = {183-193},
      doi = {10.1051/0004-6361:20021020},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002A%26A...393..183B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Merand:2005,
   author = {{M{\'e}rand}, A. and {Bord{\'e}}, P. and {Coud{\'e} du Foresto}, V.
	},
    title = "{A catalog of bright calibrator stars for 200-m baseline near-infrared stellar interferometry}",
  journal = {\aap},
   eprint = {astro-ph/0412251},
 keywords = {catalogs, stars: fundamental parameters, techniques:, interferometric, instrumentation: interferometers},
     year = 2005,
    month = apr,
   volume = 433,
    pages = {1155-1162},
      doi = {10.1051/0004-6361:20041323},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005A%26A...433.1155M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonneau:2006,
   author = {{Bonneau}, D. and {Clausse}, J.-M. and {Delfosse}, X. and {Mourard}, D. and 
	{Cetre}, S. and {Chelli}, A. and {Cruzal{\`e}bes}, P. and {Duvert}, G. and 
	{Zins}, G.},
    title = "{SearchCal: a virtual observatory tool for searching calibrators in optical long baseline interferometry. I. The bright object case}",
  journal = {\aap},
   eprint = {astro-ph/0607026},
 keywords = {instrumentation: high angular resolution, instrumentation: interferometric, stars: fundamentals parameters, catalogs, astronomical database: miscellaneous},
     year = 2006,
    month = sep,
   volume = 456,
    pages = {789-789},
      doi = {10.1051/0004-6361:20054469},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006A%26A...456..789B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanBelle:2008,
   author = {{van Belle}, G.~T. and {van Belle}, G. and {Creech-Eakman}, M.~J. and 
	{Coyne}, J. and {Boden}, A.~F. and {Akeson}, R.~L. and {Ciardi}, D.~R. and 
	{Rykoski}, K.~M. and {Thompson}, R.~R. and {Lane}, B.~F. and 
	{PTI Collaboration}},
    title = "{The Palomar Testbed Interferometer Calibrator Catalog}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0711.4194},
 keywords = {binaries: general, catalogs, infrared: stars, instrumentation: high angular resolution, instrumentation: interferometers, stars: fundamental parameters, stars: imaging, techniques: high angular resolution, techniques: interferometric},
     year = 2008,
    month = may,
   volume = 176,
      eid = {276-292},
    pages = {276-292},
      doi = {10.1086/526548},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJS..176..276V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
